Bridging the Human to Robot Dexterity Gap through Object-Oriented Rewards

Training robots directly from human videos is an emerging area in robotics and computer vision. While there has been notable progress with two-fingered grippers, learning autonomous tasks for multi-fingered robot hands in this way remains challenging. A key reason for this difficulty is that a policy trained on human hands may not directly transfer to a robot hand due to morphology differences. In this work, we present HuDOR, a technique that enables online fine-tuning of policies by directly computing rewards from human videos. Importantly, this reward function is built using object-oriented trajectories derived from off-the-shelf point trackers, providing meaningful learning signals despite the morphology gap and visual differences between human and robot hands. Given a single video of a human solving a task, such as gently opening a music box, HuDOR enables our four-fingered Allegro hand to learn the task with just an hour of online interaction. Our experiments across four tasks show that HuDOR achieves a 4x improvement over baselines. Code and videos are available on our website, https://object-rewards.github.io.

==> background.tex <==
\section{Background}
\LP{Remove}

% \method{} builds on several technical ideas in constrastive learning and optimal-transport imitation:

% \subsection{Constrastive Self-Supervised Learning}
% \label{sec:infonce}
% Self-supervised learning (SSL) seeks to learn compact representations for high-dimensional observations, such as images, to be used in downstream tasks. Contrastive methods for SSL seek to move representations between ``positive'' samples close together while moving ``negative'' samples further from one another. 

% InfoNCE~\cite{oord2019representation} is a commonly used loss function employed in contrastive learning that distinguishes positive and negative pairs based on their density ratio. For an observation and its positive pair $o_t, o_t^+$ and set of $n$ negative observations $\mathcal{D}=\{o_1, \ldots, o_n\}$, resulting in latents $z_t, z_t^+$ and $\{z_1, \ldots z_n\}$, the loss is defined as:
%  \begin{equation}
% \mathcal{L}_\text{NCE}(z_t, z_t^+, \{z_1, \ldots z_n\}) =
% -\mathbb{E}_{\mathcal{D}}\left[\log{\frac{h(z_{t}, z_t^+)}{\sum_{i=1}^n h({z}_{t}, {z}_i)}}\right]
% \label{eq:cpc}
% \end{equation}
% where $h(x,y)=\exp(x\cdot y)$.
% Maximizing this loss causes the model to assign higher probabilities to positive pairs while pushing apart negative, resulting in discriminative representations. 

\subsection{Optimal-Transport Imitation Learning}
\label{sec:ot}
We aim to learn an autonomous policy from expert demonstrations in imitation learning. This can be achieved through either offline behavior cloning (BC)~\cite{bc}, where observations are mapped to lower-dimensional actions using various architectures during training, or through inverse reinforcement learning (IRL)~\cite{few-irl-papers}, where demonstrations are used to compute a reward function.

Recent works~\cite{haldar2022watch, haldar2023teach} leverage optimal transport to infer a reward function that aligns the robot's trajectory with the expert's trajectory and then learn an online policy to mimic the expert demonstration. This policy is trained using reinforcement learning (RL) optimizers to maximize the computed reward.

Formally, let the expert trajectory be denoted as $\mathcal{T}_e = \{o_1^e, \ldots, o_T^e\}$ and the robot trajectory as $\mathcal{T}_r = \{o_1^r, \ldots, o_T^r\}$. A pairwise cost matrix, $C$, can be constructed, where each entry $C_{ij}$ represents the cost of aligning $o_i^e$ with $o_j^r$. The optimal transport algorithm is applied to find the transport plan $\mu^*$ that best aligns the expert and robot trajectories, where $\mu^*_{ij}$ corresponds to the match score between the $i$th expert observation and the $j$th robot observation. The optimal transport reward is then calculated as:

\[
r^{\text{OT}}(o_t^r) = - \sum_{t'=1}^{T}C_{t,t'}\mu^*_{t,t'}
\]

This formulation allows for time-invariant behavior comparisons. If $\mathcal{T}_r$ perfectly matches $\mathcal{T}_e$, the cost would be zero, thereby maximizing the reward. If the observations are images, the OT reward can be calculated on image representations $\{z_1^e, \ldots, z_T^e\}$ and $\{z_1^r, \ldots, z_T^r\}$ retrieved from an encoder, rather than on the raw observations.
